On Partly Overloaded Spreading Sequences with Variable Spreading Factor

Future wireless communications systems are expected to support multi-service operation, i.e. especially multi-rate as well as multi-level quality of service (QoS) requirements. This evolution is mainly driven by the success of the Internet of Things (IoT) and the growing presence of machine type communication (MTC). Whereas in the last years information in wireless communication systems was mainly generated or at least requested by humans and was also processed by humans, we can now see a paradigm shift since so-called machine type communication is gaining growing importance. Along with these changes we also encounter changes regarding the quality of service requirements, data rate requirements, latency constraints, different duty cycles et cetera. The challenge for new communication systems will therefore be to enable different user types and their different requirements efficiently. In this paper, we present partly overloaded spreading sequences, i.e. sequences which are globally orthogonal and sequences which interfere with a subset of sequences while being orthogonal to the globally orthogonal sequences. Additionally, we are able to vary the spreading factor of these sequences, which allows us to flexibly assign appropriate sequences to different service types or user types respectively. We propose the use of these sequences for a CDMA channel access method which is able to flexibly support different traffic types.

==> Chapter/Chapter2_5-requirements.tex <==
\section{Requirements and System Parameters}
As already mentioned, wireless industrial communication systems are expected to provide at least comparable performance to wire-line systems. In the following, we aim to shortly depict the requirements and system parameters of a wireless industrial communication system for the use in a closed-loop control application. 
\subsection{Reliability and Latency}
A target packet error rate of $10^{-9}$ is assumed as ultra-reliable, for example in \cite{Osman.2015}. This is, of course, only possible if adequate channel coding, such as forward error correction (FEC), is applied. For end-to-end latency a maximum delay of $1$ ms is required to serve fast control processes (up to $1$ kHz update frequency) in real time. This allows a delay budget of $500$ $\mu$s for one UL and DL transmission respectively yielding to a maximum transmission time of approximately $100$ $\mu$s \cite{Johansson.}. Regarding both constraints, it seems impossible to make use of any retransmission schemes for real-time transmissions. We expect, that closed-loop wireless industrial communication systems will not only consist of transmissions with real-time requirements, but will also have transmissions of best-effort quality. This  best-effort traffic on the other hand could use a retransmission scheme within its channel in the code domain. In table \ref{tab:requirements}, the requirements of a closed-loop wireless industrial communication system for real-time as well as best-effort transmissions is depicted.
\begin{table}[h]
\caption{Requirements of Closed-Loop-Control Wireless Industrial Communication Systems}
\begin{tabular}{l|l|l}
\textbf{Parameter} 						 & \textbf{Real-time}  & \textbf{Best-Effort}\\
\hline
Packet Error Rate (PER) 			 & $10^{-9}$												& application dependent\\
Latency [ms]									 & 0.5-10														& 10 - 50\\
Maximum number of users 			 & 128															& 128\\
Payload size [bit]						 & 48 - 1024												& 120 - 2048\\
Coverage [m]									 & several 10												& several 10\\
Automatic Repeat Request (ARQ) & No																& Yes\\
\end{tabular}
\label{tab:requirements}
\end{table}

%\begin{figure*}[ht]
	%\centering
		%\includegraphics[width=\textwidth]{figures/signal_processing_chain.jpg}
	%\label{fig:signal_processing_chain}
%\end{figure*}
\subsection{Topology of a Closed-Loop Wireless Communication System}
\label{fig:LLWCS}
For the general system setup one central node is considered which is referred to as the access point (AP) in the following and carries out the network management of the cell. The users, which are transceiver nodes connected to sensors and/or actuators, share each a direct link with the AP respectively yielding a starlike topology according to Fig. \ref{fig:system_arch}.
\begin{figure}[ht]
	\centering
		\includegraphics[width=\columnwidth]{figures/arch.pdf}
	\caption{Topology of a Low Latency Wireless Communication System}
	\label{fig:system_arch}
\end{figure}
Due to the tight delay requirements in wireless industrial communication systems, other topologies such as meshed networks are not feasible. Users receive or transmit application data from sensors or actuators via their dedicated links to the AP which may be connected to backend devices such as conventional industrial fieldbus controllers or application servers via industrial ethernets.
